fAIlureNotes: Supporting Designers in Understanding the Limits of AI Models for Computer Vision Tasks

To design with AI models, user experience (UX) designers must assess the fit between the model and user needs. Based on user research, they need to contextualize the model's behavior and potential failures within their product-specific data instances and user scenarios. However, our formative interviews with ten UX professionals revealed that such a proactive discovery of model limitations is challenging and time-intensive. Furthermore, designers often lack technical knowledge of AI and accessible exploration tools, which challenges their understanding of model capabilities and limitations. In this work, we introduced a failure-driven design approach to AI, a workflow that encourages designers to explore model behavior and failure patterns early in the design process. The implementation of fAIlureNotes, a designer-centered failure exploration and analysis tool, supports designers in evaluating models and identifying failures across diverse user groups and scenarios. Our evaluation with UX practitioners shows that fAIlureNotes outperforms today's interactive model cards in assessing context-specific model performance.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> scratch.tex <==






\paragraph{(3) Failure analysis and recovery}
Eva moves on to the last step, the failure analysis and recovery.
On the left, she sees all her persona cards, each with an image, name, and description. Again, Eva can toggle between different personas by clicking on a persona card. She can also toggle between models helping her to compare model performance if she had more than one model uploaded. Generally, the disaggregated failure metrics provide Eva with quantitative performance metrics to assess how well the AI model performs for her user groups (D1). For example, Eva sees how many objects were correctly detected (CD) versus how many were misclassified (FD), missed (MD), or unnecessarily detected (UD). For each case, she sees the occurrence's total number and relative percentage. 
The next column helps Eva assess how well the model's distribution covers her users' needs. She sees the number and percentage of experienced in-distribution (ID) and out-of-distribution (OOD) cases. This information helps Eva decide if she and her team may need to retrain the model on new classes. In the third column of the disaggregated failure metric section, Eva finds a quantitative overview of all warnings: Failing to detect (FTD), critical quality of boxes (CQB), and critical quality of score (CQS). The first warning appears when the model is not able to detect any object while the last indicates that the model's confidence score lies below a certain threshold (e.g., 95\%) \\
The following section (Failure synthesis and recovery) helps Eva synthesize her failure exploration findings and derive design considerations. 







\hari{the outline looks good. Next step is to expand and flesh out each point into paragraphs}
•	ML technology blindness is a challenge for UX designers. Without an understanding of the capabilities and more importantly the limitations (i.e., when the model could fail), it can be difficult for designers to deliver usable ML-powered experiences.
•	Unlike conventional human-centered design in which human needs inform system development, ML software teams are increasingly working with pre-trained models as a starting point. \hari{I would start with this and then connect it to your previous point}
•	Often times these models are indented to support general-purpose tasks such as object detection or language translation without consideration of specific application contexts.
•	Consequently, designers need to explore the model and contextualize model failures in user research which includes the needs of diverse stakeholders and their use contexts. [specific knowledge]
•	This understanding is necessary for (1) assessing the fit for the envisioning AI experience, (2) deriving design requirements such as error handling and recovery strategies, and (3) in some cases supplying requirements and assessment criteria to engineering teams to modify existing models to fit the application purpose.
•	Unfortunately, beyond high-level overviews supported by model documentation (e.g., model cards), we lack the tools to support the integration of user research with model understanding.
1.	In this work, we introduce <system name> ("Limits"), a failure analysis too \hari{We should decide if its a failure analysis tool or model explorer for designers} and workflow for designers to acquire design <values> by aligning user requirements with pre-trained models.

\hari{V1: Pre-trained models offer a useful starting point for designing AI experiences. Services such as Hugging Face~\cite{} allow AI developers to democratize machine learning capabilities by making pre-trained models accessible to application designers. The designer's task is then to explore these models to understand their ``capabilities and limitations'' to find one that best fits their application needs. For instance, imagine designing a language-learning application that allow learners to take pictures of everyday objects to learn their names. The designer has access to tens of models with varying characteristics and performance. Existing documentation such as Model Cards provide a generalized summary about the model's intended use, but are insufficient to assess fit. AI failures are often tied to specific user data and use contexts such poor voice transcription for children's speech, failure to recognize text in a foreign language, or detect partially occluded objects, etc. How should designers assess which model might best fit their design vision? How can can they understand the limitations of the model?}

\hari{V2: To design with AI, the designer must understand the ``capabilities and limitations'' of the AI they are working with. Documentation such as model cards offer a starting point by providing a high level overview of the model's intended use and limitations. However, they do not convey specific data and contexts in which the model can fail. How should designers explore the... For instance,  }

We began our semi-structured interview by talking about the practitioner’s role in their company and their team affiliation. We then asked them to describe an AI-based application they helped design and inquired if they experienced AI-related failures during the design process. Questions included: How did you discover the failure case? How did you fix the problem? Did you work with engineers to fix the problem?
We were also interested in the methods, processes, and tools that UX experts generally use to learn about the capabilities and limitations of the AI model. Questions included: How do you know about the capabilities of a pre-trained AI model? What methods and tools do you use to detect or prevent AI failures? How can we make the process of finding failure cases more efficient? All interview questions can be found in the supplemental materials. 
In the last 20-30 minutes of the interview, participants were presented with a specific use case and a pre-trained AI model of the Hugging Face \cite{} platform. The use case was an AI-powered language learning app that helps beginners learn single words in a foreign language. To do this, users take a picture with their smartphone camera and pass it to an object detector. The computer vision system automatically detects all objects in a scene and shows or reads out the words for these objects in the foreign language. We chose Hugging Face’s pre-trained DETR model \cite{} as our model. The model included a model card with details about the architecture and intended uses, as well as details about the training procedure and evaluation results. Hugging Face also provides a hosted inference API that allows users to test the model by uploading images. We used this API and asked participants to explore the capabilities and limitations of the DETR model. Participants were encouraged to use Google to search for images of objects they wanted to test the model on. Often we encouraged participants to find challenging but realistic samples to “break” the model. Depending on the practitioner’s speed, they tested between three and ten images during the exercise. The insights from this process helped us derive design guidelines for \system.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE: Demography of study participants
\begin{table}[t!]
\begin{tabular}{ l l l }

\Xhline{1.0pt}  
\textbf{ID} & \textbf{Role} & \textbf{Work Experience in AI} \\
\Xhline{1.0pt} 

1 & UX Researcher & 10 \\
\hline
2 & UX Researcher & 4 \\
\hline
3 & Senior UX Researcher & 1 \\
\hline
4 & Lead Product Manager & 6 \\
\hline
5 & Product Manager & 5 \\
\hline
6 & Product Manager & 8 \\
\hline
7 & Senior UX Researcher & 4 \\
\hline
8 & Product Manager AI for Design & 4 \\
\hline
9 & UX Researcher & 6 \\
\hline
10 & AI Product Manager & 4 \\

\Xhline{1.0pt}  
\end{tabular}
\caption{Demography of Study Participants}
\label{table:demography}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In the interest of the session time, we also provided users with a persona and three data samples that a colleague supposedly collected during an earlier Wizard of Oz study.


\subsubsection{Analysis}
Around 600 minutes of the interviews were recorded and transcribed using a third-party service. For data analysis, we relied on an inductive coding approach \cite{saldana2015}. The first five interviews were open coded by the first author to create the initial codebook. The resulting codebook consisted of 86 codes. The remaining five sessions were then coded using this codebook. In another round, the author classified the annotated codes into several categories using MURAL \cite{}. All authors then reviewed the categories in multiple sessions and discussed the thematic relevance to the topic of successful AI failure discovery. In several cycles, we identified the most important emergent themes. We refined the themes until all categories and subtopics were covered and no new topics emerged. We used memos to summarize findings across transcripts and as a basis for internal discussion \cite{birks2008}.

\subsection{Existing methods for AI failure discovery}
The goal for product designers is to proactively identify AI failures before they harm users and avoid or at least mitigate them when they do occur. Such failures often arise from a mismatch between user expectations and the behavior of the AI model. In our preliminary study, we found that the ideal way to detect AI failures is through methods that incorporate both realistic user and model behavior. We found that such proactive approaches are rarely used because they are resource intensive. Instead, UX practitioners, particularly the product managers we interviewed, often rely on reactive approaches in which the first version of the AI-enabled solution is rolled out relatively quickly. User feedback is then used to iteratively improve the user experience and model (fine-tuning, re-training, online training). Most methods that UX practitioners use to anticipate AI-related failures during earlier product development do not involve the AI model and therefore cannot realistically test the model's behavior. Figure \ref{figure:overview} provides an overview of our findings. In the following, we elaborate on the approaches UX practitioners used to detect and avoid AI failures.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\graphicspath{ {./figures} }
\includegraphics[scale=0.5]{failure_discovery}
\caption{Overview of existing failure discovery methods}
\end{figure}
\label{figure:overview}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Proactive methods that include both the user and the AI model are expensive but fruitful}
Methods that anticipate AI errors before deployment (Proactive) and test realistic user and AI behavior (AI and User) are rarely used because they tend to be resource intensive. 
P8 said: \say{I think one of the biggest challenges is we can create really cool demos with a static sort of like walkthrough prototype, but making reactive prototypes to test with users is highly expensive}. Interestingly, some participants used such approaches and described them as highly efficient in detecting AI failure cases. We describe three of them in more detail: (1) building specialized tools, (2) making use of human-in-the-loop, and (3) setting up semi-realistic environments to test the AI with users in the field.
P1 and his team developed several tools in addition to the actual AI-driven product. He described these tools in the context of building a computer vision-based system for a large consumer products company (CPG) that would help sales agents to accurately arrange their shelves in a store. To collect high-quality data, he and an engineer developed a special \say{UI that helped guide the [store] agent to create nicely tiled images [of their shelves]}. In later phases, they built a specialized debugging tool that allowed them to test the model behavior with users in the wild. \say{So we created this debugging tool [...] and then we would go into the store with our functional prototype and take images of the store shelves and look at the corrections that came back and kind of debug what [the AI] was getting right and wrong, and then try to figure out why. Looking at different layers of the tech stack to figure out where the problem was arising}. The development of these tools took a lot of time and effort. Moreover, they were developed specifically for the problem P1 and his team were trying to solve and could not be applied to other computer vision cases without considerable effort. P1 later explained that this was only possible because his partner had a background in user research and engineering that allowed him to switch effortlessly between user requirements and model behavior. After building the first version of the actual AI-driven product, he described how he set up semi-realistic environments to test it with users. \say{We set up multiple store shelves in our facilities. So we could try out [the product] within that environment, which is semi-realistic. Like the lighting was a bit different. Distances and things like that were a little bit off. We bought real store shelving. We bought like a few thousand dollars worth of products and loaded up the shelves}. Semi-realistic environments differ from soft launches such as a beta launch in that users are invited to test the product and each session is carefully monitored. A similar approach is to launch the AI-powered application to real end users, but have a human tester review the model in each case (human-in-the-loop). P6 said, \say{so if it comes to our ability to know how well our machine works, we heavily relied on human-in-the-loop}. Staff was hired and trained, and \say{every time they changed or flagged [the algorithm] we'll keep track of all of those edits. And we will then use that to both manually revisit and learn what are patterns for avoiding these mistakes in the future} (P6). Again, this is a fairly expensive process that does not allow for much scalability. However, the main advantage of all these approaches is that failures can be fixed before they harm users. In addition, UX experts can discover many failure cases and types with these approaches because they test both user and model behavior under realistic conditions.




 However, application designers use these pre-trained models at a stage where they often lack use-case-specific data or labels for a systematic and context-specific assessment.


Such an assessment may also be critical for large self-supervised models that can solve various ML tasks in different industries. 



To address this challenge, we conceptualize a designerly model exploration process centered around users. \system encourages designers to explore AI models for various user scenarios, probe models to their limitations, and brainstorm recoveries for groups of failures in early design phases even before crafting the user interface. 





For example, large language models such as OpenAI's GPT-3 \cite{brown2020} or its open access counterpart BLOOM conduct text summary, completion or language translation. However, application designers use these pre-trained models at a stage where they often lack use-case-specific data or labels for a systematic and context-specific assessment. Future research could build tools that support model assessment for self-supervised models to facilitate a responsible way of commercialization.

\paragraph{AI failure detection is often reactive rather than proactive}
Several practitioners indicated they take a more reactive approach to AI-related failure detection. Some practitioners said they would first implement a rule-based system and then use lessons learned to derive specific requirements for a learning system. Many product managers would also resort to soft launches, where a minimum viable product is introduced to a select group of beta users. P5 illustrated this approach by saying: \say{We'll try to see what is the fastest proof of concept I can build for probably a very small group of users that still represent the broad group of users … Getting to production as fast as possible is the most important part in building ML models because it's great that you have all this training data, but reality is very, very different}. Accelerated product deployments help practitioners not only evaluate whether the system behavior meets user requirements under realistic conditions (AI and user), but also collect more data. This data can then be used to fine-tune an existing model or completely re-train the model if needed. Alternatively, the data can be fed directly back into the model to improve its performance (online learning). A quick soft or full launch can be useful when little is at stake (low-stake situation) because the AI-powered solution is being tested under realistic conditions. Additionally, UX experts can quickly analyze the user behavior of different target groups, identify borderline cases, or detect model deficiencies. However, this approach also has drawbacks. First, the approach is reactive rather than proactive. \say{So usually our changes are reactive rather than anticipating what the pitfalls might be} (P8).
As practitioners improve the user experience and model behavior iteratively based on implicit or explicit user feedback, this approach places the burden of failure detection entirely on the user. P5 noted: \say{So if [users] encounter any issue or problem, they can feel free to reach out in the early days, what was mainly manual}.
Furthermore, it can be quite difficult to detect AI failures. While qualitative user testing (in semi-virtual environments) creates a direct feedback loop between users and UX experts, this is not the case in a soft launch. Instead, UX experts often have to interpret quantitative customer success or product metrics. \say{And the big part of that is us detecting [AI failure cases] with enough analytics so that we can hear back and say, okay, this is a moment in time, not as a timestamp, but as an action in which the user left or the user, you know, [he/she] gave us a thumbs down or, the user just reacted to us with a signal. So all the little perhaps annoying, thumbs down and thumbs up are some of the few interactions in the wild that we can have with users} (P8). 
Lastly, most product decisions have always been made at this stage, and a soft launch is mainly seen as an opportunity to tweak final features and fix minor bugs. P8 explains: \say{I don't think we have a sort of like a really good playground or internal sand sandbox … So a low stakes refining product is kind of what the need is because … once you do a limited test, then it's a different thing and most of the decisions are made, and mainly you're looking for bugs and sort of like minor refinements and ‚yes‘, and ‚nos‘ before it ships}.


\paragraph{Most proactive methods do not include the AI model}
Before a product launch, the qualitative research methods that help detect AI-related failures of all kinds typically do not include tests of AI behavior. In the early stages of product development, practitioners often relied on their imagination to anticipate AI failures ex-ante (no user and no AI). For example, several of our participants conducted technology-related research on potential AI errors before designing the initial user interface. One participant even claimed that reading science fiction would help him think about specific AI failures in the future. \say{And finally, maybe this sounds fun to you, but we also spend a lot of time reading science fiction. Trying to see what other people are predicting about possible failure to AI… just how people are imagining that this could fail} (P4).
When sketching high-level user journeys or experience maps, practitioners often brainstormed failure cases for each step in the journey. Similarly, thinking about user context helped UX practitioners come up with potential model-related issues while discussing the impact of typical failure cases from the user's perspective. P5 demonstrated this with the example of a fictional spam classifier: \say{What are the problems when it comes to false positives and false negatives. So what's the impact of those things. And so a false negative is I see spam in my inbox and there are ways that you'd want to then fix that. [...] And then false positives though, I think those are the ones that you want to really like to worry about because that means that I'm pointing something that I really do want to have access to into the spam folder}. All of these methods can help anticipate AI-related failures at a very early stage in the design process. However, due to the highly theoretical nature of such approaches, it is difficult to predict specific unpredictable cases arising from the unexpected user or AI behavior.
In the later stages of the design phase, our UX practitioners relied on radical user-centricity to ensure that the AI-powered solution would meet user requirements (No user and No AI). By becoming intimately familiar with the user's domain, they were able to better understand AI's shortcomings and discover edge cases. P1 said: \say{Like we actually became kind of like experts in the domain. And we were very aware of these kinds of edge case areas that were harder to distinguish. So we could actually provide fixes in those situations}.
Most user research methods did not consider the model behavior. To simulate AI behavior, practitioners relied on either role-playing or Wizard-of-Oz studies. P7, a product manager, said: \say{Usually what I do is I'll partner with a designer and we will create a high fidelity prototype that I will Wizard of Oz. So I will pretend to be the model for the purpose of qualitative discovery}.
Previous work \cite{browne2019} has shown that Wizard of Oz prototyping helps product designers bring a human-centered design approach to the development of AI-powered technical experiences. Recently, however, studies have found that Wizard of Oz prototypes can be overly optimistic \cite{begel2020} and designers may have difficulty making the same mistakes that an AI would make \cite{jansen2022}. P4 also reported mixed results:
\say{Uh, I think sometimes it worked well sometimes not that well because it's difficult [...] to test some parts of [the AI-powered product]. And also when you test just one feature that is embedded in a very large flow, you are getting just a lot of noise instead of real information, real data. So what, the more complex the flow was, the less data or quality data we used to get}.


\paragraph{Limited involvement of UX professionals in AI engineering practices to mitigate errors}
The UX professionals in our study clearly distinguished between their work and the engineering practices used to mitigate AI errors. Despite acknowledging the importance of AI engineering practices (No User but AI), such as conducting technical failure analysis, selecting appropriate value functions, reviewing performance metrics, or AI-specific quality assurance testing (QA), UX practitioners themselves had limited involvement in these processes. P5 said: \say{Most of the time I would work with a machine learning engineer that would be the person that would actually do the work, right. So I'm a product manager. And what I would do is we would have discussions about what types of scenarios I wanted to enable and what types of failure modes I wanted to avoid. And then they would do work to understand how this model may fail}. 
When teams took an "AI-first" or "a priori" approach \cite{windl2022}, in which the AI model is trained before the user interface is created, the designer's role was to test whether the model behavior matches user expectations. \say{I usually come in when the model is already created and I test whether it meets [the users'] goals or not} (P9).
In a "post-hoc" approach, where the interface is created before the model is trained and when the model and interface are created in parallel, the designer's role was more important. UX experts needed to steer the AI engineering process towards solving a real problem from the user's perspective. P7 said: \say{It's a natural reflex as a user researcher to try to find the person in the truest context possible. To have the model solve a real problem or a real need. And because that's where the failure lies - when [the model] is not actually solving things that are in context and that actually solve a problem. That's the big weakness from the lens of a user researcher. Right. And so it's about trying to mitigate that in advance so that you don't spend a whole bunch of time training your model against something that doesn't actually make an impact}.
In essence, UX practitioners ensured that model behavior matched what users would expect in a given context. However, designers had limited direct involvement in technical processes such as conducting failure analysis or cross-checking performance metrics. Similar to the work of \cite{subramonyam2022b, yang2018}, we found designers often do not engage in technical aspects of AI projects. In other words, there is a clear separation of concerns between design and AI engineering. To share user information across boundaries, designers relied on use cases, user scenarios, and AI personas. Alternatively, engineers communicated the model's capabilities and limitations to UX designers in the form of videos or technical demonstrations during one-on-one meetings. P5 said: \say{And basically, I had seen videos from engineers of how it would work, right. So they'll take little snippets of videos to show what is happening on their machine. And I would give feedback based on that}, whereas P8 said: \say{And after that, once we know that there's a level of maturity and there's a demo, what we'll do is we'll set up a technical deep dive. And the purpose of that deep dive is to focus on a particular use case or use cases}.

\subsection{Design Considerations for Failure Exploration Tools}
By observing ten practitioners probing a pre-trained model for failure cases, we identified three important aspects for supporting better failure exploration tools: User-centricity, variety of failures, iterative and contrastive exploration, and guidance and active support.

\paragraph{User-centricity}
User --> Context --> Inputs --> Failure \\
Many practitioners took a similar approach when asked to examine the pre-trained model for failures. They first inquired about a particular user group. Imagining the user in a particular context then helped the practitioners think of specific samples the user may feed to the AI. They then searched the Internet for appropriate images and tested the model on those images. P8 demonstrated this by imagining a science student during a semester abroad: \say{If for example, I was to study abroad in Berlin and I was doing a physics course and I wanted to know what a particular object was called, then translating would be really useful}. She then looked for a picture of a solar system. The model incorrectly classified the "planets" as "balls." Other participants took a similar user-centered approach, imagining a tourist exploring the landscape of Paris, a fashion designer wanting to learn about different types of shoes, or a man in Japan going to a store to learn about different kitchen appliances. Practitioners would then conduct multiple iterations of this procedure with the same or different target subjects in mind. In each case, the context and needs of the user served as a starting point for testing the model for failures. The overall suitability of the model depended on how well it covers all relevant user scenarios. P9 explains, \say{As UX researchers, we try to ask first whom we are building it for, who's going to use it. So that might help you to narrow down: Is there any model built for that specific type of user? Are we building it for a child or the elderly? [...] And we then select the model based on that}. These findings suggest that failure exploration tools should be built in a user-centered way. More specifically, such tools \textbf{should allow UX practitioners to test the model for different user groups and contexts (D1)}.

\paragraph{Variety of AI failures}
In the context of supervised learning, a model-related error is defined as a discrepancy between the prediction of the AI model and the ground truth. Since UX experts see the world through the eyes of the end user, the term error is defined more broadly to include not only errors within the distribution but also out-of-distribution and context errors. P3 imagined a tourist in France who wanted to find out about various objects in a café. She inserted a picture of a croissant, which the model incorrectly classified as a "cat" because it had not been trained on the class "croissant." In other words, the class "croissant" is not in the distribution of the model. Similarly, she imagined a language learner interested in the foreign word for "milk" or "coffee," but the model generalized both cases to "cup." P6 also had trouble with objects outside the model's distribution when the model misclassified a picture of ice cream as a "teddy bear." P4, on the other hand, imagined that someone wanted to learn the plural. He first looked for a picture of a single apple and later for multiple apples and entered them into the model. P4 was disappointed that the model could not cover this context, even though it was a realistic case for a person who had just started to learn a new language. From these findings, we conclude that \textbf{AI tools for failure exploration should allow UX professionals to test the model for a variety of failures beyond in-distribution errors (D2)}.

\paragraph{Iterative failure exploration}
Many of our participants iteratively examined the AI for failures, using previous images to help practitioners form new hypotheses. P5 wanted to see if the model was capable of recognizing different ethnicities and inserted an image with 24 faces. 
Originally, he wanted to test the model on people of color because he had heard that computer vision models had difficulty in this area. In fact, the model could not recognize a black person in the top row. The model also failed to recognize a man who had many facial tattoos. P5 then tested the model specifically for people with facial tattoos. In this case, a simple coincidence inspired P5 to think of another group that may be more prone to be misclassified by the model. More generally, our participants were often interested in the "why". P5 said, \say{I think the question I would ask myself would be: Why aren't these two faces working}? In many cases, they took a contrastive and iterative approach to learn more about why the model failed to predict certain objects. For example, when P8 found that the model incorrectly classified the planets in our solar system as "balls," she hypothesized that the reason for this error might be similarity in shape. This prompted her to search for other round objects such as chemical molecules. We conclude that to gain a sufficient understanding of the limitations of a model, \textbf{failure exploration tools should follow an iterative approach that allows practitioners to test new or slightly modified hypotheses effortlessly (D3)}.

\paragraph{Guidance and active support}
Testing a pre-trained model for failures was an unusual task for many of our participants. P4 said, \say{So this was something new to me because usually when I use these models is when they are already implemented for testing in the real environment. So to test the model was something new for me}. When conducting the interview, we provided ample guidance to the participants throughout the process, which they appreciated.  \say{So I really liked it. However, I just haven't worked with this Hugging Face website before [and] it wasn't natural to me to think about how to test it out. So I appreciated your guidance there} (P8).
We also found that UX practitioners sometimes made incorrect assumptions about the reasons for an experienced failure. For instance, due to a lack of technical understanding, participants had difficulty understanding out-of-distribution errors. We asked one participant specifically why the model was unable to detect flowers. She hypothesized that it could be due to a lack of contrast with the surrounding background or that the model had difficulty with organic objects. This fact is consistent with previous literature addressing the issue of UX practitioners' technical blindness to their design work \cite{dove2017, qian2020, subramonyam2022a}. \textbf{Therefore, failure exploration tools should guide UX professionals throughout the process and actively promote understanding of different failure modes (D4)}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Failure-Driven Design in AI with a focus on Computer Vision}
\label{theory}

\hari{I propose moving this to the system section}

Similar to the work of \cite{avizinienis2004, honig2018}, we define an \textit{AI failure} as a degraded state of an AI system that causes a deviation in behavior from an ideal or correct service to an incorrect or unideal service. Whether or not the behavior of an AI system is correct or incorrect in a given context depends on the system’s function which is ``what the system is intended to do'' from a human point of view. 
Our study focuses on AI-related failures that commonly arise in computer vision systems. 
We focus on failures that directly affect the end-user instead of external stakeholders or engineers. We only included failures that occur in a single human-AI interaction \textit{local failures} and excluded the ones that require several interactions, such as mental model breakdowns \textit{global failures}. \textit{Failure-driven-design} implies anticipating the ways an AI system may fail (\textit{failure mode}) and finding effective actions to prevent or recover from failure (\textit{failure recovery}). Our separation into failure modes and failure recovery was inspired by work in risk management, more specifically by the ``Failure Mode and Effects Analysis (FMEA)'' \cite{liu2013, dhillon1992}.  

\subsection{Failure Modes in Computer Vision} 
Previous work has shown that UX practitioners tend to be unaware of the range of failures possible with their AI-powered system \cite{hong2021}. This led researchers to develop different taxonomies of AI-related failures \cite{hong2021, buschek2021}. To develop a taxonomy of typical failure modes that occur in computer vision systems we first reviewed existing taxonomies for the field of natural language processing \cite{hong2021} and Human-AI co-creative systems \cite{buschek2021}. We then collected an initial set of failure modes by reviewing earlier work on human failures from the field of psychology and cognitive science. The work of \cite{bahaei2019} followed a similar approach and crafted a taxonomy of failures for augmented reality technologies. We revisited human failure types from Norman's taxonomy \cite{norman1980, norman1981}, Rasmussen's taxonomy \cite{rasmussen1982}, Reason's taxonomy \cite{reason2016} as well as the HFACS taxonomy \cite{shapell2000} which is based on Reason. We also integrated more recent failure categorizations, such as a taxonomy for human driving \cite{stanton2009}. The first author collected all failure modes in a long table. From this long list of failures, we then selected the ones that are relevant for computer vision technology. Through several meetings and discussions, we developed the categorization presented in table \ref{table:failure_modes}. Lastly, we did a final check and walked through a range of computer vision tasks to see if we covered most failure cases. More specifically, we looked at the tasks of binary image classification, multi-class classification, object detection, single-object tracking, multiple-object tracking, semantic segmentation, instance segmentation, panoptic segmentation, video object segmentation, deep metric learning, and image generation. This led to some final adjustments in our final definitions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% TABLE: Taxonomy of failures in computer vision
% \textbf{Table \ref{table:1}: A Taxonomy of failures in computer vision.}
\begin{table}[p!]
\begin{tabular}{ p{1.8cm} p{2.2cm} p{5cm} p{6cm}  }

\Xhline{1.0pt}  
\textbf{System level} & \multicolumn{2}{c}{\textbf{Failure Mode}} & \textbf{Example Autonomous Driving}  \\
\Xhline{1.0pt} 

% ATTENTION
\multirow{5}{0pt}{Attention and sensing} & Missed or delayed attention & System fails to detect a triggering event or responds too late to be useful. & Motion detection system fails to trigger camera or triggers camera system too late.
\\
\cline{2-4}
& False input & System fails because it is unable to process a particular input. & System is fed lidar data but can only process camera data. \\
\cline{2-4}
& Critical quality input & System fails because of quality issues with respect to the input. & System fails because it was fed a blurry image. \\
\hline


% OBSERVATION
\multirow{13}{0pt}{Observation} & False observation & Computer vision system generates output error.  & Object detection system misclassifies a pedestrian as another car (in-distribution error).  \\
\cline{2-4}
& Failing to observe & Computer vision system is unable to provide an output due to a limitation of the system. & Object detection system is unable to detect a cow because the system has not been trained on this particular class (out-of-distribution error).  \\
\cline{2-4}
& Incomplete observation & Computer vision system misses certain visual information.
 & Object detection system detects many objects correctly but misses a pedestrian in a frame. \\
\cline{2-4}
& Critical quality output & The output of the computer vision system bears intolerable uncertainty or quality issues. & The top two classes of an object detection system have almost the same certainty score. \\
\cline{2-4}
& Violation & Computer vision system’s output stands in conflict with ethical standards, rules, or regulations.  & Object detection system classifies the eyes of an Asian person to be closed.
 \\
\hline

% INTERPRETATION AND DECISION MAKING
\multirow{6}{0pt}{Interpretation \\ and \\  decision making} & False decision & System misjudges the situation and maps it to the wrong category of action. & Vehicle trajectory prediction underestimates the speed of another vehicle and wrongly decides not to break. \\
\cline{2-4}
& Failing to decide & System fails to interpret the situation and cannot map the observation to any known action category. & System encounters an edge case such as observing a motorboat on a follower and fails to make any decision.  \\
\hline

% ACTION
\multirow{15}{0pt}{Action} & Failing to act & System fails in executing the desired action. & Vehicle does not break due to a problem with the electronics.  \\
\cline{2-4}
& Mistimed action & System acts according to the user's needs but at the wrong point in time. & Vehicle breaks not fast enough to prevent an accident. \\
\cline{2-4}
& Too much AI
 & From a human perspective, the system enters the territory of the user or automates too much of the process. & Autonomous driving assistant takes over but the human driver would prefer driving in this given situation. \\
\cline{2-4}
& Limited AI & From a human perspective, the system provides too little involvement in the process to provide value.  
 & Autonomous driving system supports human drivers with steering and acceleration (L1) but the driver expects it also to monitor the environment (L3).  \\
 \cline{2-4}
& Inappropriate action (context error) & System works as intended but the behavior of the system stands in conflict with the needs, goals or preferences of its user in a given context.
 & Autonomous vehicle speeds to be able to cross a traffic light in time but fails to take the passenger's driving anxiety into consideration. 
 \\

\Xhline{1.0pt}  
\end{tabular}
\caption{A Taxonomy of Failures in Computer Vision.}
\label{table:failure_modes}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We differentiate between three different layers: an input layer, a computer vision layer, and an action layer as many computer vision systems are constructed this way. We list several potential failure modes for each level and also provide an illustrative example for each focusing on the use case of autonomous driving. It is important to mention that not all failure modes will apply to every vision-empowered product. Instead, the taxonomy is designed to alert a designer or engineer to a wide range of potential failures but requires the user to select and interpret the different failure modes for their specific context.

\begin{comment}
\subsection{Failure Effects}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\graphicspath{ {./figures} }
\includegraphics[scale=0.5]{failure_effects}
\caption{Failure Effects}
\end{figure}
\label{figure:failure_effects}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Computer vision systems can harm humans in many different ways. We were interested in categorizing the types of harm they can cause and for that analyzed 179 incidents of the AI incidents database \cite{mcgregor2020}. The first author put every incident on a virtual sticky note in MURAL before classifying them into categories. We find that AI systems can cause harm on three different levels: harming the individual, harming specific communities, or harming our societal structures. For each level, we found four to five types of harm. The categories were inspired by earlier work in cyber attacks \cite{agrafiotis2016}and psychology \cite{grossman2014}. We provide an example for each category in figure ~\ref{figure:failure_effects}.\\

The AI incidents that our categorization is based on not only include computer vision cases but also other technologies such as natural language processing or robotics. However, we found a computer vision example in each category. We are aware that the AI incidents database may lean towards more extreme stories with a large focus on big technology companies such as Google, Facebook, or Amazon. Our theoretical work is by no means holistic, but we hope this categorization of failure effects can serve as a starting point for future studies. 
Commented code
\end{comment}

\subsection{Failure Recovery}
\label{failure_recovery}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\graphicspath{ {./figures} }
\includegraphics[scale=0.5]{failure_recovery}
\caption{Failure Recovery}
\end{figure}
\label{figure:failure_recovery}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There are several practices that UX designers can follow to recover from AI-related failures. Often the topic is coined ``graceful failure''. We were interested in collecting best practices of failure recovery strategies for UX designers. We analyzed three different guidelines on AI experience design (Google’s People + AI guidebook \cite{pair2019}, Microsoft’s Guidelines on Human-AI Interaction \cite{amershi2019} and Apple’s Human Interface Guidelines for Machine Learning \cite{apple2019}. The first author captured every item on a virtual sticky note in MURAL. This approach helped us to identify eight commonly applied recovery strategies that we present in table \ref{figure:failure_recovery}.
% Figure
We acknowledge that there are many more ways to prevent AI failures and errors. There are best practices in engineering for choosing the right value function, network architecture, or performance metrics. Not to mention training the AI on high-quality data or conducting technical error analysis for model failure. For this study we focus on failure recoveries on a UX/UI level. 

\begin{comment}
\subsubsection{Failure Effects}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\graphicspath{ {./figures} }
\includegraphics[scale=0.5]{failure_effects}
\caption{Failure Effects}
\end{figure}
\label{figure:failure_effects}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Computer vision systems can harm humans in many different ways. We were interested in categorizing the types of harm they can cause and for that analyzed 179 incidents of the AI incidents database \cite{mcgregor2020}. The first author put every incident on a virtual sticky note in MURAL before classifying them into categories. We find that AI systems can cause harm on three different levels: harming the individual, harming specific communities, or harming our societal structures. For each level, we found four to five types of harm. The categories were inspired by earlier work in cyber attacks \cite{agrafiotis2016}and psychology \cite{grossman2014}. We provide an example for each category in figure ~\ref{figure:failure_effects}.\\

The AI incidents that our categorization is based on not only include computer vision cases but also other technologies such as natural language processing or robotics. However, we found a computer vision example in each category. We are aware that the AI incidents database may lean towards more extreme stories with a large focus on big technology companies such as Google, Facebook, or Amazon. Our theoretical work is by no means holistic, but we hope this categorization of failure effects can serve as a starting point for future studies. 
Commented code
\end{comment}



\hari{todo: focus more on failures, failures are hard to understand}


\hari{envisioning product}

\hari{first draft of intro, let me know your thoughts. I will get back to it tomorrow}
\vera{Nitpicking, feel free to ignore. I feel there misses a sentence about designers must work with AI but impossible to do it from scratch, instead of jumping to off-the-shelf directly. }Off-the-shelf AI models are a valuable design resource for crafting AI experiences. Services such as \textit{Hugging Face}~\cite{hugging} host numerous models trained in a variety of AI capabilities, including object detection, language translation, and speech recognition. To design with such pre-trained models, the first step is for designers to explore the capabilities and limitations of the models by considering diverse users and their contexts of use~\cite{yang2018,subramonyam2021}. For example, imagine designing a photo-based language learning application, one that identifies objects in images in a new language. Ideally, such an application should work in a variety of contexts, including a tourist walking through the city center, buying groceries, and an immigrant building their vocabulary. By considering several different object detection models, the designer must (1) understand the model behavior and when and why it might fail, (2) evaluate the model's performance for different user groups and scenarios, (3) select a model \vera{...if there are multiple candidates...} that can produce the best performance in real-world use, and (4) generate design considerations for an optimal user experience based on model limitations. 

Unfortunately, designers currently lack the means to explore AI models in a human-centered way. In characterizing AI as a `design material,' prior work recommends designers to build their understanding of AI models by connecting AI material properties to end-user needs, their expectations, and their reception of designed AI experiences~\cite{}. There are several challenges to building this understanding. First, given the vast input space for general-purpose AI models, discovering unknown unknowns about when the model might fail is a challenge for designers. Exploration requires examining the behavior of the model across a range of inputs and their variations. Second, pre-trained models are indented to support general-purpose tasks without consideration of specific application contexts. Hence, documentation such as model cards, while providing an overview of training, performance, and intended use, is not effective at assessing model fit for a specific application contexts. AI failures are often tied to specific user data and use contexts such as poor voice transcription for children's speech, failure to recognize text in a foreign language, or detect partially occluded objects, etc.  Third, AI material exploration for designerly understanding requires both probing models with different inputs to observe output performance and also synthesizing design insights through such exploration \vera{i feel this sentence is a bit of getting ahead of ourselves? Is it obvious to readers that it requires probing with different inputs? maybe cite some papers can help... } Existing GUI based model APIs are limited to testing one input at a time and do not lend themselves well to designers workflow. 

\hari{TODO: talk about golden path and failure exploration challenges}
\vera{not sure if it is very relevant to this study. In the other paper we make a point that error does not equate with failure, and not equate with user risk/harms. There can be no error but still UX failures (output sentence is too long). There can be errors but if in one scenario the user risk/harms/frequency is low you can also let it go}

Consequently, designers approach AI experience design with a partial (or incomplete) understanding of model behavior. Through our formative need-finding interviews, we learned that designers and product managers rely largely on wizard-of-oz simulations to explore model behavior rather than directly interact with model APIs. Proactive approaches to model understanding are uncommon, as they are considered to be resource-intensive.  Instead, designers respond to model failures observed during controlled deployment. This approach is problematic as both upstream and downstream changes can be costly. In the previous example, the designer may fail to understand that the model does not recognize certain object classes or multiple objects in scene, or that it consistently fails when used in scenarios typical to relocating to a new country.  Practitioners need model exploration tools that are application and end-user centered, support the discovery of a range of AI failures that may require design mediation, and the exploration is guided. To address these needs, we investigate \textit{how can we support designerly understanding of the capabilities and limitations of pre-trained AI models?} 

In this work, we introduce \system, a model (AI design material) exploration and analysis tool. \system implements an integrated workflow for guided model exploration, failure assessment, and UX design synthesis. Starting with user personas or groups and example input data generated through user research, the designer can explore how the model behaves in a disaggregated manner. As shown in Figure~\ref{fig:teaser}, the designer can select an input (in this case an image for language learning) and annotates it with ground truth. Calling the model API returns the model output for the input image highlighting any mismatch between end-user expectations about model behavior and actual behavior. Further \system generates suggestions for alternative inputs to either address model failures or further explore unknown unknowns. Through iterative exploration the designer can compare behavior across different models, examine performance of models for different personas, and synthesis design considerations based on observed model failures. 

\system provides a designerly way to explore AI models by incorporating requirements from user research into the exploration process. Our interactive interface and scaffolding features enables designers to understand different types of model errors and proactively discover unknown unknowns to design AI experiences. \system enables a necessary first step in working with pre-trained AI models as a design material. Our key contributions include (1) design considerations for model exploration derived from need-finding interviews with practitioners, (2) \system --- an GUI instantiation of the design consideration for computer vision tasks, and (3) results from evaluation of our model exploration workflow. 



